Causal Dantzig: fast inference in linear structural equation models with hidden variables under additive interventions

Causal inference is known to be very challenging when only observational data are available. Randomized experiments are often costly and impractical and in instrumental variable regression the number of instruments has to exceed the number of causal predictors. It was recently shown in Peters et al. [2016] that causal inference for the full model is possible when data from distinct observational environments are available, exploiting that the conditional distribution of a response variable is invariant under the correct causal model. Two shortcomings of such an approach are the high computational effort for large-scale data and the assumed absence of hidden confounders. Here we show that these two shortcomings can be addressed if one is willing to make a more restrictive assumption on the type of interventions that generate different environments. Thereby, we look at a different notion of invariance, namely inner-product invariance. By avoiding a computationally cumbersome reverse-engineering approach such as in Peters et al. [2016], it allows for large-scale causal inference in linear structural equation models. We discuss identifiability conditions for the causal parameter and derive asymptotic confidence intervals in the low-dimensional setting. In the case of non-identifiability we show that the solution set of causal Dantzig has predictive guarantees under certain interventions. We derive finite-sample bounds in the high-dimensional setting and investigate its performance on simulated datasets.

==> crvsiv1 <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Tue Mar 28 13:45:59 2017
\begin{table}[ht]
\centering
\begin{tabular}{rlll}
  \hline
 & $n = 20 $ & $ 50 $ & $ 100 $ \\ 
  \hline
causal Dantzig & 0.46$\pm$0.41 & 0.03$\pm$0.01 & 0.01$\pm$0 \\ 
  ivreg & 0.07$\pm$0.01 & 0.02$\pm$0 & 0.01$\pm$0 \\ 
   \hline
\end{tabular}
\caption{Mean square error for varying $n$. Instrument is not weak.} 
\label{crvsiv1}
\end{table}


==> crvsiv2 <==
% latex table generated in R 3.4.3 by xtable 1.8-2 package
% Fri Apr  6 19:43:43 2018
\begin{table}[ht]
\centering
\begin{tabular}{rlll}
  \hline
 & $n = 20 $ & $ 50 $ & $ 100 $ \\ 
  \hline
causal Dantzig & 24.05$\pm$90.75 & 0.03$\pm$0 & 0.01$\pm$0 \\ 
  ivreg & 36634.21$\pm$161096.94 & 4244.29$\pm$15557.82 & 1862.7$\pm$8171.14 \\ 
   \hline
\end{tabular}
\caption{Mean square error for varying $n$. The instrument is weak, but \emph{causal Dantzig} can leverage changes in variance.} 
\label{crvsiv2}
\end{table}


==> latexpand <==
#!/usr/bin/perl
# Inspired by latexpand by D. Musliner, University of Michigan
# 2012, 2013, 2014, 2015, 2016, 2017: Matthieu Moy <git@matthieu-moy.fr>
# BSD License

use strict;
use Cwd;
use Getopt::Long;
use IO::Handle;
use File::Spec;

my $TEXINPUTS = $ENV{'TEXINPUTS'};
if (!$TEXINPUTS) { $TEXINPUTS = getcwd(); }

my $verbose;
my $keep_comments;
my $keep_includes;
my $empty_comments;
my $help;
my $long_help;
my $output;
my $explain;
my $show_graphics;
my $graphics_extensions = ":.pdf:.png:.jpg:.eps";
my $expand_usepackage;
my $expand_bbl;
my $fatal;
my $version;
my $makeatletter;
my $inside_import;

GetOptions (
	'h' => \$help,
	'help' => \$long_help,
	'verbose|v' => \$verbose,
	'keep-comments' => \$keep_comments,
	'keep-includes' => \$keep_includes,
	'empty-comments' => \$empty_comments,
	'output|o=s' => \$output,
	'explain' => \$explain,
	'show-graphics' => \$show_graphics,
	'graphics-extensions' => \$graphics_extensions,
	'expand-usepackage' => \$expand_usepackage,
	'expand-bbl=s' => \$expand_bbl,
	'fatal' => \$fatal,
	'version' => \$version,
        'makeatletter' => \$makeatletter,
) or pod2usage_wrapper(2);
version() if $version;
pod2usage_wrapper(0) if $help;
pod2usage_wrapper(-exitstatus => 0, -output => \*STDOUT, -verbose => 2) if $long_help;

sub pod2usage_wrapper
{
	# Like pod2usage, but fall back to a simpler implem in case
	# pod2usage can't be found.
	if  (eval {require Pod::Usage;1;} ne 1) {
		print "Please install perldoc and Pod::Usage to get proper help.\n";
		my $started = 0;
		open (my $in, '<', "$0") or die $!;
		while (<$in>) {
			if ($started) {
				print;
			}
			if (/^__END__$/) {
				$started = 1;
			}
		}
	} else {
		Pod::Usage->import();
		pod2usage(@_);
	}
}

sub get_version
{
	# $VERSION's value will be substituted by 'make dist', but the
	# next line won't (the string has to be broken to avoid it).
	my $VERSION = 'v1.4-1-gb32a776';
	if ($VERSION eq '@LATEXPAND' . '_VERSION@') {
		my($vol,$dir,$file) = File::Spec->splitpath($0);
		chdir($dir);
		$VERSION = `git describe --tags HEAD 2>/dev/null`;
	}
	if ($VERSION eq '') {
		$VERSION = '<unknown version>';
	}
	$VERSION =~ s/^\s+|\s+$//g;
	return $VERSION;
}

sub version
{
	print "latexpand version ". get_version() .".\n";
	exit(0);
}

my $nl = "";
if ($empty_comments) {
	$nl = "%\n";
}

if ($output && $output ne "-") {
	open (my $OUTPUT, '>', "$output") or die $!;
	STDOUT->fdopen(\*$OUTPUT, 'w') or die $!;
}

sub say
{
	if ($verbose) {
		print STDERR "$_[0]";
	}
}

my $makeatletter_found;
my $in_preamble;

foreach my $file (@ARGV)
{
	say "processing $file\n";
	$makeatletter_found = 0;
	$in_preamble = 1;
        $inside_import = "";
	process_file($file, "  ");
}

sub process_file
{
	my $file = shift;
	my $prefix = (shift || "");
	my $in_comment = 0;
	open(my $FILE, "<", $file) or die "could not open input file '$file'\n";
	my $commented_newline = 0;
	while (my $line = <$FILE>) {
		if ($line =~ /^[ \t]*\\endinput/) {
			$line =~ s/(\\endinput.*)\n/% $1/;
			$in_comment = 1;
			process_line($line, $prefix, \$commented_newline);
			last;
		}
		process_line($line, $prefix, \$commented_newline, $file);
		if ($line =~ /^%.*[^\n]\z/ || $line =~ /[^\\]%.*[^\n]\z/) {
			# file ends with a comment not ending with a newline
			print "\n";
		}
		# Garbage at end of line after \end{document} is
		# ignored by LaTeX, but we don't allow anything before
		# to avoid e.g. \verb|\end{document}| from terminating
		# the file.
		if (!$keep_comments && $line =~ /^[ \t]*\\end\{document\}/) {
			last;
		}
	}
	close($FILE);
	return $in_comment;
}

sub process_line
{
	my ($line, $prefix, $commented_newline, $file) = @_;
	$_ = $line;
	if ($$commented_newline && /^\s*$/) {
		# Deal with:
		#
		# Line 1 % comment
		#
		# Line 2
		#
		# The newline after Line 1 is commented, but we still
		# want a new paragraph. We strip the comment together
		# with its newline, but re-add a newline to chnge
		# paragraph here if needed:
		print "\n";
	}
	$$commented_newline = 0;
	# Consider \makeatletter only in preamble, because we do want
	# to warn on \someCommand{\makeatletter\command@with@arobase}.
	if ($in_preamble && /^[^%]*\\makeatletter/) {
		$makeatletter_found = 1;
	}
	if ($in_preamble && /^[^%]*\\makeatother/) {
		$makeatletter_found = 0;
	}
	if (!$makeatletter && !$makeatletter_found
	    && (my ($command) = /^[^%]*(\\[[:alpha:]]*@[[:alpha:]]*)/)) {
		print STDERR "Warning: command $command containing @ found in\n";
		print STDERR "Warning: $file.\n";
		print STDERR "Warning: consider using --makeatletter if the result is not compilable.\n";
	}
	unless ($keep_comments) {
		if (!$empty_comments) {
			# Include \n in pattern to avoid matching
			# comments at end of files

			# remove comments + whitespace-only lines completely
			if (s/^\s*%.*\n//) {
				$$commented_newline = 1;
			}

			# remove only the comment if the line has actual content
			if (s/([^\\])%.*\n/$1/) {
				$$commented_newline = 1;
			}
		}
		# Apply the "empty comments" treatment unconditionally
		# for end-of-files comments not matched above (it
		# doesn't harm to keep an empty comment sometimes, but
		# it may harm to leave a real comment if the goal was
		# to strip them).
		s/^%.*$/%/;
		s/([^\\])%.*$/$1%/;
	}

	unless ($keep_includes) {
		if (my ($before, $ignored, $full_filename, $after)
		    = /^(([^%]|[^\\]%)*)\\include[{\s]+(.*?)[\s}](.*)$/) {
			$full_filename = find_tex_file($full_filename . ".tex");
			if ($full_filename) {
				say $prefix . "Found include for file: $full_filename\n";
				print $before . $nl;
				print '\clearpage{}' . $nl;
				print "% start include $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end include $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				print '\clearpage{}' . $nl;
				print $nl . $after . "\n";
				$_ = "";
			}
		} elsif (my ($before, $ignored, $full_filename, $after)
			 = /^(([^%]|[^\\]%)*)\\input[{\s]+(.*?)[\s}](.*)$/) {
                        if ($inside_import) {
                              $full_filename = $inside_import . $full_filename;
                        }
			$full_filename = find_tex_file($full_filename, ":.tex");
			if ($full_filename) {
				say $prefix . "Found input for file: $full_filename\n";
				print $before . $nl;
				print "% start input $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end input $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				if ($after =~ /[^\s]/) {
				    # LaTeX produces this space, so let's do it also
				    print " " . $nl . $after . "\n";
				} else {
				    print " ";
				}
				$_ = "";
			}
		} elsif (my ($before, $ignored, $dir, $full_filename, $after)
			 = /^(([^%]|[^\\]%)*)\\(?:sub)?import[{\s]+(.*?)[\s}][{\s]+(.*?)[\s}](.*)$/) {
                        if ($explain) {
                              print "% dir " . $dir ."\n";
                              print "% full_filename " . $full_filename ."\n";
                              print "% after " . $after ."\n";
                              print "% inside_import $inside_import\n";
                        }
                        $full_filename = $dir . $full_filename;
                        if ($inside_import) {
                              $full_filename = $inside_import . $full_filename;
                        }
                        print "% cat(inside_import,dir,full_filename) " . $full_filename ."\n" if ($explain);
			$full_filename = find_tex_file($full_filename, ":.tex");
			if ($full_filename) {
				say $prefix . "Found input for file: $full_filename\n";
				print $before . $nl;
				print "% start input $full_filename\n" if ($explain);
                                my $previous_import_dir = $inside_import;
                                $inside_import = $inside_import . $dir;
				my $in_comment = process_file($full_filename, $prefix . "  ");
                                $inside_import = $previous_import_dir;
				if ($explain) {
				    print " % end input $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				if ($after =~ /[^\s]/) {
				    # LaTeX produces this space, so let's do it also
				    print " " . $nl . $after . "\n";
				} else {
				    print " ";
				}
				$_ = "";
			}
		} elsif (my ($before, $ignored, $args, $full_filename, $after)
			 = /^(([^%]|[^\\]%)*)\\includegraphics[\[\s]+(.*?)[\s\]][{\s]+(.*?)[\s}](.*)$/) {
                        if ($explain) {
                                print "% inside_import " . $inside_import ."\n";
                                print "% before " . $before ."\n";
                                print "% ignored " . $ignored ."\n";
                                print "% args " . $args ."\n";
                                print "% full_filename " . $full_filename ."\n";
                                print "% after " . $after ."\n";
                        }
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                                print "$before\\includegraphics[$args]{$full_filename}$after\n";
                                $_ = "";
                        }
		} elsif (my ($before, $ignored, $args, $full_filename, $after)
			 = /^(([^%]|[^\\]%)*)\\lstinputlisting[\[\s]+(.*?)[\s\]][{\s]+(.*?)[\s}](.*)$/) {
                        if ($explain) {
                                print "% inside_import " . $inside_import ."\n";
                                print "% before " . $before ."\n";
                                print "% ignored " . $ignored ."\n";
                                print "% args " . $args ."\n";
                                print "% full_filename " . $full_filename ."\n";
                                print "% after " . $after ."\n";
                        }
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                                print "$before\\lstinputlisting[$args]{$full_filename}$after\n";
                                $_ = "";
                        }
		}
	}
	if ($expand_usepackage) {
		# Don't bother with before and after text, we just require the
		# usepackage to be alone on its line.
		if (my ($package_name) = /^\s*\\usepackage\{([^\}]*)\}\s*(%.*)?$/) {
			my $full = find_file($package_name . ".sty", $TEXINPUTS);
			if ($full) {
				say $prefix . "Found package file: $full\n";
				process_file($full, $prefix . "  ");
				$_ = "";
				# Forget about any commented newline
				# before the \usepackage:
				$$commented_newline = 0;
			} else {
				say $prefix . "Not including external package $package_name\n";
			}
		}
	}
	if ($expand_bbl) {
		if (my ($before, $bib_name, $after)
			 = /^(.*)\\(?:bibliography|bibselect)\{([^\}]*)\}(.*)$/) {
			# The BBL file is not necessarily $bib_name.
			# Take it from the command-line.
			print $before . $nl;
			say $prefix . "Expanding BBL file: $expand_bbl\n";
			process_file($expand_bbl, $prefix . "  ");
			print " " . $nl . $after . "\n";
			$_ = "";
		}
	}
	if ($show_graphics) {
		if (/\\includegraphics(\[[^\]]*\])?{([^}]*)}/) {
                        my $full_filename = $2;
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                        }
			my $full = find_tex_file($full_filename, $graphics_extensions);
			say $prefix . "needs graphics file: ";
			print STDERR "$full\n";
		}
	}
	if (/^[ \t]*\\begin\{document\}/) {
		$in_preamble = 0;
		if ($makeatletter) {
			print '\makeatletter' . $nl;
		}
	}
	print;
}

# search $1 in $TEXINPUTS, with possible extensions in $2
sub find_tex_file
{
	my $file = shift;
	my $extensions = (shift || ":");
	foreach my $ext (split(':', $extensions, -1)) {
		my $full = find_file_global($file . $ext);
		if ($full) {
			return $full;
		}
	}
	if ($fatal) {
		die "ERROR: Could not find file [$file]\n";
	} else {
		print STDERR "Warning: Could not find file [$file]\n";
		return;
	}
}

sub find_file_global
{
	my $file = shift;
	if (open(my $fh, "-|", "kpsewhich", $file)) {
		my $full = <$fh>;
		chomp($full);
		close($fh);
		if ($full) {
			return $full;
		}
	}
	return find_file($file, $TEXINPUTS);
}

sub find_file
{
	my ($file, $path) = @_;
	if (File::Spec->file_name_is_absolute($file)) {
		if (-e "$file" && ! -d "$file") {
			return $file;
		} else {
			return;
		}
	}
	foreach my $dir (split(':', $path)) {
		if (-e "$dir/$file" && ! -d "$dir/$file") {
			return("$dir/$file");
		}
	}
	return;
}


__END__

=head1 NAME

latexpand - Flatten LaTeX file by expanding \include and \input, ... and  remove comments

=head1 SYNOPSIS

latexpand [options] FILE...

=head2 Options:

	--verbose        show what's going on
	--keep-comments  don't strip comments (comments are lines
                         starting with %, and anything below
                         \end{document})
	--empty-comments keep empty comments (i.e. % at end of lines) for clarity
	--keep-includes  don't expand \input and \include directives
	--expand-usepackage
	                 Expand \usepackage{...} directives if the
	                 corresponding .sty file is found in
	                 $TEXINPUTS (or the current directory if
	                 $TEXINPUTS is not set)
	--expand-bbl FILE
	                 Expand the bibliography by inlining FILE
	                 (should be a *.bbl file)
	--help           this help message
	--output <file>, -o <file>
	                 generate output in <file>
	--explain        generate explanatory comments in output
	--show-graphics  show included graphics
	--graphics_extensions
	                 colon-separated list of possible graphics extensions
	                 (used by --show-graphics to find the actual graphics files)
	--fatal          Die in case a file can't be found.
	--makeatletter   Insert a \makeatletter in the preamble. In some
	                 rare cases it may break your document, but it
	                 may help fixing bad interactions between
	                 @-commands and inclusion (see BUGS section).

=head1 USES

The most common use of latexpand is to simplify distribution of source
LaTeX files, typically to satisfy the requirement of editors and
archival sites (springer, arXiv.org, ...) who force the authors to
submit sources. One does not necessarily want to submit sources with
comments, and uploading a document made of several files including
each other is a bit painful. By default, latexpand answers both
problems by outputing a single LaTeX file that contain no comment.

=head1 GETTING LATEXPAND

The latest version of latexpand is available here:

  https://gitlab.com/latexpand/latexpand

Versions are uploaded to ctan.org from time to time:

  http://www.ctan.org/pkg/latexpand

=head1 BUGS

Please, report bugs on the issue tracker on the project site:

  https://gitlab.com/latexpand/latexpand/issues

=head2 Known bugs

=head3 Verbatim

latexpand currently ignores \begin{verbatim} ... \end{verbatim}, and
will therefore process any \include, \input, ... directives that
appear within verbatim environments (while it shouldn't).

LaTeX comments inside verbatim environments are also incorrectly
stripped. You can use --keep-comments as a workaround to avoid this.

=head3 Comment environment

It would be nice to remove code between \begin{comment} and
\end{comment} too if \usepackage{comment} is used.

Code like

	foo%
	\begin{comment}

will produce the incorrect

	foo\begin{comment}

A workaround is to use --empty-comments when such tricky usage of the
comments package is done.

=head3 \makeatletter and use with transfig/xfig with \scalebox{}

If \input{} or \include{} appears as argument to a command, and the
file included contains \makeatletter, then after expansion, the
\makeatletter and the @-command appear as argument to the command,
which is forbidden because the argument is parsed (and the @-command
badly tokenized) before being executed.

This happens with

	\scalebox{ \input{file-generated-by-xfig.pdf_t} }

Workaround: add \makeatletter before the scalebox manually in your
code, like

        \makeatletter{}
	\scalebox{ \input{file-generated-by-xfig.pdf_t} }
        \makeatother{}

In the case of xfig generated files, it is necessary only for the
first occurence.

A more brute-force workaround is to use latexpand --makeatletter.

=head1 SEE ALSO

Instructions to include only the relevant .bib items (french):

https://lacl.fr/~caubert/notes/portabilite-du-tex.html#dependances

=head1 VERSION

This is latexpand version v1.4-1-gb32a776.


==> nicosimAcombined <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Mar 27 22:47:16 2017
\begin{table}[ht]
\centering
\begin{tabular}{rllll}
  \hline
 & $n = 50 $ & $ 100 $ & $ 500 $ & $ 1000 $ \\ 
  \hline
Coverage & 0.93$\pm$0.01 & 0.95$\pm$0.01 & 0.96$\pm$0.01 & 0.96$\pm$0.01 \\ 
  Average length & 65.79$\pm$2918.53 & 4.11$\pm$602.53 & 0.27$\pm$0.62 & 0.18$\pm$0.01 \\ 
  Coverage ICP & 0.92$\pm$0.01 & 0.84$\pm$0.01 & 0.42$\pm$0.02 & 0.3$\pm$0.03 \\ 
   \hline
\end{tabular}
\caption{The first two rows contain actual coverage and average length of confidence intervals of \emph{causal Dantzig} for the first variable in SEM (A) of equation~\eqref{eq:simulatins}. The last row contains the actual coverage of ICP in these settings. The nominal coverage is $0.95$ for causal Dantzig and at least $0.95$ for ICP. For small sample sizes, the variance is relatively large. As discussed in Section~\ref{sec:high-dim}, regularization can be helpful in these settings.} 
\label{simulations1length}
\end{table}


==> nicosimB <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Mar 27 22:52:11 2017
\begin{table}[ht]
\centering
\begin{tabular}{rllll}
  \hline
 & $n = 50 $ & $ 100 $ & $ 500 $ & $ 1000 $ \\ 
  \hline
Coverage & 0.95$\pm$0.01 & 0.95$\pm$0.01 & 0.96$\pm$0.01 & 0.96$\pm$0.01 \\ 
  Average length & 11354.75$\pm$2776.95 & 57.27$\pm$28842.69 & 0.69$\pm$7.28 & 0.39$\pm$3.73 \\ 
   \hline
\end{tabular}
\caption{Actual coverage and average length of confidence intervals for first variable in SEM (B) of equation~\eqref{eq:simulatins} with causal Dantzig. The nominal coverage is 0.95.} 
\label{simulations2}
\end{table}

